Sequential Convex Programming for Optimal Line of Sight Steering in Agile Missions

The trend toward onboard autonomy and spacecraft minimization present significant potential for advances in efficient Line of Sight management by making optimal use of the limited torque resources available. At SENER Aeroespacial, we are implementing AOCS algorithms capable of providing agility in different observation scenarios in which the exploitation of the resources is fundamental for the mission success. In this contribution, we present an in-house optimization toolbox for onboard guidance, the SENER Optimization Toolbox, and we propose its use for online attitude guidance of an agile space-craft using Control Moment Gyroscopes. We propose different optimization schemes based on Sequential Convex Programming aiming for reducing the computational burden for real-time implementations. The results highlight the potential for performance improvements when making use of embedded optimal control for fast slew maneuvers: with proposed schemes, we find solutions that implicitly manage singularities and are up to 12.2% faster than classical bang-bang maneuvers while increasing the smoothness of the trajectories to minimize the excitation of flexible modes.

==> MATLAB_figures/BenchmarkBoxplot.tex <==
\begin{tikzpicture}
  \begin{axis}
    [
        xlabel = {\# iterations},
        width=12cm,
        height=5cm,
        ytick={1,2,3,4},
        yticklabels={\emph{Chain}, \emph{Diesel}, \emph{Crane 1}, \emph{Crane 2}},
    ]
    \addplot+[mark=*,
    boxplot prepared={
      median=7,
      upper quartile=10,
      lower quartile=7,
      upper whisker=11,
      lower whisker=6
    },
    ] coordinates {};
    \addplot+[mark=*,
    boxplot prepared={
      median=9,
      upper quartile=10,
      lower quartile=9,
      upper whisker=11,
      lower whisker=8
    },
    ] table [row sep=\\,y index=0] {
        data\\    
        12\\ 
        12\\
        12\\
        12\\
        12\\
        12\\
        13\\
        13\\
        14\\
        };
    \addplot+[mark=*,
    boxplot prepared={
      median=114,
      upper quartile=124,
      lower quartile=107,
      upper whisker=149,
      lower whisker=90
    },
    ] table [row sep=\\,y index=0] {
        data\\    
        150 \\
        151 \\
        151 \\
        153 \\
        153 \\
        154 \\
        154 \\
        154 \\
        154 \\
        154 \\
        155 \\
        155 \\
        155 \\
        155 \\
        155 \\
        156 \\
        156 \\
        159 \\
        159 \\
        161 \\
        163 \\
        165 \\
        169 \\
        };
        \addplot+[mark=*,
            boxplot prepared={
              median=32,
              upper quartile=33,
              lower quartile=31,
              upper whisker=35,
              lower whisker=29
            },
            ] table [row sep=\\,y index=0] {
                36 \\
                36 \\
                36 \\
                37 \\
                37 \\
                37 \\
                37 \\
                37 \\
                37 \\
                37 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                38 \\
                39 \\
                39 \\
                39 \\
                40 \\
                40 \\
                40 \\
                40 \\
                40 \\
                40 \\
                41 \\
                41 \\
                42 \\
                42 \\
                42 \\
                42 \\
                43 \\
                43 \\
                43 \\
                43 \\
                43 \\
                44 \\
                44 \\
                44 \\
                44 \\
                44 \\
                45 \\
                45 \\
                45 \\
                45 \\
                45 \\
                45 \\
                46 \\
                46 \\
                46 \\
                46 \\
                46 \\
                46 \\
                47 \\
                47 \\
                47 \\
                48 \\
                48 \\
                48 \\
                48 \\
                49 \\
                49 \\
                50 \\
                50 \\
                50 \\
                51 \\
                52 \\
                52 \\
                53 \\
                53 \\
                53 \\
                53 \\
                55 \\
                57 \\
                58 \\
                59 \\
                59 \\
                59 \\
                59 \\
                59 \\
                59 \\
                59 \\
                59 \\
                59 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                60 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                61 \\
                62 \\
                62 \\
                62 \\
                62 \\
                62 \\
                62 \\
                63 \\
                64  \\
                };
        
  \end{axis}
\end{tikzpicture}
